Rotationally symmetric plabic graphs and the Lagrangian Grassmannian

We introduce the totally nonnegative Lagrangian Grassmannian $\rm{LG}_{\geq 0}^R (n,2n)$, a new subset of the totally nonnegative Grassmannian consisting of subspaces isotropic with respect to a certain bilinear form $R$. We describe its cell structure and show that each cell admits a representation by a rotationally symmetric (not necessarily reduced) plabic graph. Along the way, we develop new techniques for working with non-reduced plabic graphs.

==> tikz/abcd-graph.tex <==
\newcommand{\xx}{1.52}
\begin{tikzpicture}[scale = \graphscale]
        \draw[line width=\graphcircle,opacity=0.3] (0,0) circle (3);
        \draw[line width=\graphline,blue] (0.93,0.93) -- (-0.93,0.93);
        \draw[line width=\graphline,blue] (0.93, -0.93) -- (-0.93,-0.93);
        \draw[line width=\graphline,blue] (0.93, 0.93) -- (0.93, -0.93);
        \draw[line width=\graphline,blue] (-0.93,0.93) -- (-0.93, -0.93);
        \draw[line width=\graphline,blue] (0.93,0.93) -- ({3 * cos(45)}, {3 * sin(45)});
        \draw[line width=\graphline,blue] (-0.93,0.93) -- ({-3 * cos(45)}, {3 * sin(45)});
        \draw[line width=\graphline,blue] (-0.93,-0.93) -- ({-3 * cos(45)}, {-3 * sin(45)});
        \draw[line width=\graphline,blue] (0.93,-0.93) -- ({3 * cos(45)}, {-3 * sin(45)});
        
        \bdot{{3*cos(45)}}{{3*sin(45)}};
        \bdot{{-3*cos(45)}}{{3*sin(45)}};
        \bdot{{-3*cos(45)}}{{-3*sin(45)}};
        \bdot{{3*cos(45)}}{{-3*sin(45)}};
        \wdot{\xx}{-\xx};
        \wdot{-\xx}{\xx};
        \wdot{0.93}{0.93};\bdot{-0.93}{0.93};\wdot{-0.93}{-0.93};\bdot{0.93}{-0.93};
        
        \node [above right] at ({3*cos(45)},{3*sin(45)}) {1};
        \node [below right] at ({3*cos(45)},{-3*sin(45)}) {2};
        \node [below left] at ({-3*cos(45)},{-3*sin(45)}) {3};
        \node [above left] at ({-3*cos(45)},{3*sin(45)}) {4};
        \small
    
        \node[above, scale = 1.5, color = red,inner sep=4pt] at (0,0.93) {$d$};
        \node[right, scale = 1.5, color = red,inner sep=4pt] at (0.93,0) {$a$};
        \node[below, scale = 1.5, color = red,inner sep=4pt] at (0,-0.93) {$b$};
        \node[left, scale = 1.5, color = red,inner sep=4pt] at (-0.93,0) {$c$};
\end{tikzpicture}

==> tikz/fixed-point-proof/F-special-case.tex <==
\newcommand{\xx}{1.4}
\begin{tikzpicture}[scale = \graphscale, baseline={(0,0)}]
    \draw[line width=\graphcircle,opacity=0.3] (0,0) circle (3);

    \draw[line width=\graphline, blue] (3,0) -- (1, 0);
    \draw[line width=\graphline, blue] (-3,0) -- (-1, 0);

    \draw[line width=\graphline, blue] ({3*cos(50)},{3*sin(50)}) arc (-50:-130:3);
    \draw[line width=\graphline, blue] ({3*cos(-50)},{3*sin(-50)}) arc (50:130:3);
    

    %the G part
    %%%%%%%


    %%%%%%

    \wdot{3}{0}; \bdot{-3}{0};
    \bdot{1}{0}; \wdot{-1}{0};
    
    
    \small
    \node [right] at ({3*cos(0)},{3*sin(0)}) {$i$};
    \node [left] at ({3*cos(180)},{3*sin(180)}) {$i+n$};
    \node at (0,2.6) {\ldots};
    \node at (0,-2.6) {\ldots};
    \normalsize
\end{tikzpicture}

==> tikz/fixed-point-proof/G-special-case.tex <==
\newcommand{\xx}{1.4}
\begin{tikzpicture}[scale = \graphscale, baseline={(0,0)}]
    \draw[line width=\graphcircle,opacity=0.3] (0,0) circle (3);

    \draw[line width=\graphline, blue] (3,0) -- (1, 0);
    \draw[line width=\graphline, blue] (-3,0) -- (-1, 0);

    \draw[line width=\graphline, blue] ({3*cos(50)},{3*sin(50)}) arc (-50:-130:3);
    \draw[line width=\graphline, blue] ({3*cos(-50)},{3*sin(-50)}) arc (50:130:3);
    

    %the G part
    %%%%%%%
    
    \draw[line width=\graphline,  red] (1,0) edge node[below] {$\boldsymbol{e = e'}$} (-1,0);


    \node[below] at (-0.4,0.9) (f) {};
    \draw[red, ->, line width=\graphcircle] (f) to[loop, in = 0, out=90,looseness=\loosns] (f);

    \node[right] at (3,2) (ff) {face $\face = \face'$};
    \draw (0.6,0.9) -- (ff);
    %\node[left] at (-3,2) (ff') {face $\face'$};
    %\draw (-0.6,0.9) -- (ff');


    %%%%%%

    \wdot{3}{0}; \bdot{-3}{0};
    \bdot{1}{0}; \wdot{-1}{0};
    
    
    \small
    \node [right] at ({3*cos(0)},{3*sin(0)}) {$i$};
    \node [left] at ({3*cos(180)},{3*sin(180)}) {$i+n$};
    \node at (0,2.6) {\ldots};
    \node at (0,-2.6) {\ldots};
    \normalsize
\end{tikzpicture}

==> tikz/fixed-point-proof/fpp-F.tex <==
\newcommand{\xx}{1.4}
\begin{tikzpicture}[scale = \graphscale, baseline={(0,0)}]
    \footnotesize
    \draw[line width=\graphcircle,opacity=0.3] (0,0) circle (3);

    \draw[line width=\graphline, blue] (0,0) ellipse (\xx cm and 1cm);

    \draw[line width=\graphline, blue] (3,0) -- (1.5 + 0.5*\xx, 0);
    \draw[line width=\graphline, blue] (-3,0) -- (-1.5 - 0.5*\xx, 0);
    \draw[line width=\graphline, blue] ({cos(90)*\xx}, {sin(90)}) -- ({2*cos(90)*\xx}, {2*sin(90)});
    \draw[line width=\graphline, blue] ({cos(70)*\xx}, {sin(70)}) -- ({2*cos(70)*\xx}, {2*sin(70)});
    \draw[line width=\graphline, blue] ({cos(110)*\xx}, {sin(110)}) -- ({2*cos(110)*\xx}, {2*sin(110)});
    \draw[line width=\graphline, blue] ({-cos(75)*\xx}, {-sin(75)}) -- ({-2*cos(75)*\xx}, {-2*sin(75)});
    \draw[line width=\graphline, blue] ({-cos(105)*\xx}, {-sin(105)}) -- ({-2*cos(105)*\xx}, {-2*sin(105)});

    \wdot{3}{0}; \bdot{-3}{0};
    \bdot{1.5 + 0.5*\xx}{0}; \wdot{-1.5 - 0.5*\xx}{0}
    \wdot{\xx}{0}; \bdot{-\xx}{0};
    
    
    \small
    \node [right] at ({3*cos(0)},{3*sin(0)}) {$i$};
    \node [left] at ({3*cos(180)},{3*sin(180)}) {$i+n$};
    \node at (0,0) {\ldots};
    \normalsize
\end{tikzpicture}

==> tikz/fixed-point-proof/fpp-G.tex <==
\newcommand{\xx}{1.4}
\begin{tikzpicture}[scale = \graphscale, baseline={(0,0)}]
    \draw[line width=\graphcircle,opacity=0.3] (0,0) circle (3);

    \draw[line width=\graphline, blue] (0,0) ellipse (\xx cm and 1cm);

    \draw[line width=\graphline, blue] (3,0) -- (1.5 + 0.5*\xx, 0);
    \draw[line width=\graphline, blue] (-3,0) -- (-1.5 - 0.5*\xx, 0);
    \draw[line width=\graphline, blue] ({cos(90)*\xx}, {sin(90)}) -- ({2*cos(90)*\xx}, {2*sin(90)});
    \draw[line width=\graphline, blue] ({cos(70)*\xx}, {sin(70)}) -- ({2*cos(70)*\xx}, {2*sin(70)});
    \draw[line width=\graphline, blue] ({cos(110)*\xx}, {sin(110)}) -- ({2*cos(110)*\xx}, {2*sin(110)});
    \draw[line width=\graphline, blue] ({-cos(75)*\xx}, {-sin(75)}) -- ({-2*cos(75)*\xx}, {-2*sin(75)});
    \draw[line width=\graphline, blue] ({-cos(105)*\xx}, {-sin(105)}) -- ({-2*cos(105)*\xx}, {-2*sin(105)});

    %the G part
    %%%%%%%
    
    \draw[line width=\graphline,  red] (1.5 + 0.5*\xx, 0) edge node[below] {$\boldsymbol{e}$} (\xx,0);
    \draw[line width=\graphline,  red] (-1.5 - 0.5*\xx, 0) edge node[below] {$\boldsymbol{e'}$} (-\xx,0);


    \node[below] at (0.5 + 0.7*\xx,0.9) (f) {};
    \draw[red, ->, line width=\graphcircle] (f) to[loop, in = 0, out=90,looseness=\loosns] (f);
    
    \node[below] at (-0.5 - 1.3*\xx,0.9) (f') {};
    \draw[red, ->, line width=\graphcircle][red, ->, line width=\graphcircle] (f') to[loop, in = 0, out=90,looseness=\loosns] (f');

    \node[right] at (3,2) (ff) {face $\face$};
    \draw (0.5 + 1.3*\xx,0.9) -- (ff);
    \node[left] at (-3,2) (ff') {face $\face'$};
    \draw (f') -- (ff');


    %%%%%%

    \wdot{3}{0}; \bdot{-3}{0};
    \bdot{1.5 + 0.5*\xx}{0}; \wdot{-1.5 - 0.5*\xx}{0}
    \wdot{\xx}{0}; \bdot{-\xx}{0};
    
    
    \small
    \node [right] at ({3*cos(0)},{3*sin(0)}) {$i$};
    \node [left] at ({3*cos(180)},{3*sin(180)}) {$i+n$};
    \node at (0,0) {\ldots};
    \normalsize
\end{tikzpicture}

==> tikz/fixed-point-proof/fpp.tex <==
\begin{center}

\begin{tabular}{ccc}

    {\input{tikz/fixed-point-proof/fpp-F}}
    &
    {%\vrule
    }
    &
    {\input{tikz/fixed-point-proof/fpp-G}}\vspace{0.2cm} \\ 
    {$F$} & & {$G$}
\end{tabular}
\end{center}
\normalsize

==> tikz/fixed-point-proof/special-case.tex <==
\begin{center}

\begin{tabular}{ccc}

    {\input{tikz/fixed-point-proof/F-special-case}}
    &
    {%\vrule
    }
    &
    {\input{tikz/fixed-point-proof/G-special-case}}\vspace{0.2cm} \\ 
    {$F$} & & {$G$}
\end{tabular}
\end{center}
\normalsize
